Counting and equidistribution in Heisenberg groups

We strongly develop the relationship between complex hyperbolic geometry and arithmetic counting or equidistribution applications, that arises from the action of arithmetic groups on complex hyperbolic spaces, especially in dimension $2$. We prove a Mertens' formula for the integer points over a quadratic imaginary number fields $K$ in the light cone of Hermitian forms, as well as an equidistribution theorem of the set of rational points over $K$ in Heisenberg groups. We give a counting formula for the cubic points over $K$ in the complex projective plane whose Galois conjugates are orthogonal and isotropic for a given Hermitian form over $K$, and a counting and equidistribution result for arithmetic chains in the Heisenberg group when their Cygan diameter tends to $0$.

==> macros_angl.tex <==
\usepackage[utf8]{inputenc}
\usepackage{amsmath,amssymb,epsfig,bbm}
\usepackage{comment}
\usepackage[dvips]{color}
\usepackage[T1]{fontenc}
%\usepackage[latin1]{inputenc}

%\usepackage[notcite,notref]{showkeys}
%\renewcommand{\theequation}{-\,\arabic{equation}\,-}
\renewcommand{\labelenumi}{{\rm (\arabic{enumi})}}

\usepackage{todonotes}
\usepackage{enumitem}
\setlist{nolistsep}

%%%%
%% Format de page
%%%%

\pagestyle{plain}
\textwidth 15cm    
\textheight 22.5cm 
\oddsidemargin 0.5cm
\evensidemargin 0.5cm
\topmargin 30pt
\headheight 0pt
\headsep 0pt
%\footheight 10pt
\footskip 20pt
   
%%%%
%% environnements theoremes
%%%%

\newtheorem{defi}{Definition}
\newtheorem{prop}[defi]{Proposition}
\newtheorem{theo}[defi]{Theorem}
\newtheorem{conj}[defi]{Conjecture}
\newtheorem{lemm}[defi]{Lemma}
\newtheorem{coro}[defi]{Corollary}
\newtheorem{rema}[defi]{Remark}
\newtheorem{exem}[defi]{Example}
\newtheorem{exems}[defi]{Examples}

\newcommand{\bdefi}{\begin{defi}}
\newcommand{\edefi}{\end{defi}}
\newcommand{\bprop}{\begin{prop}}
\newcommand{\eprop}{\end{prop}}
\newcommand{\btheo}{\begin{theo}}
\newcommand{\etheo}{\end{theo}}
\newcommand{\blemm}{\begin{lemm}}
\newcommand{\brema}{\begin{rema}}
\newcommand{\erema}{\end{rema}}
\newcommand{\bexer}{\begin{exem}}
\newcommand{\eexer}{\end{exem}}
\newcommand{\bexems}{\begin{exems}}
\newcommand{\eexems}{\end{exems}}
\newcommand{\bconj}{\begin{conj}}
\newcommand{\econj}{\end{conj}}
\newcommand{\elemm}{\end{lemm}}
\newcommand{\bcoro}{\begin{coro}}
\newcommand{\ecoro}{\end{coro}}
\newcommand{\dem}{\noindent{\bf Proof. }}
\newcommand{\rem}{\noindent{\bf Remark. }}
\newcommand{\exemp}{\medskip\noindent{\bf Example. }}

%%%%
%% fonte \cal
%%%%

\usepackage{mathrsfs}
\renewcommand\mathcal{\mathscr}


\newcommand{\A}{{\cal A}}
%\newcommand{\R}{{\cal R}}
\newcommand{\T}{{\cal T}}
\newcommand{\B}{{\cal B}}
\renewcommand{\L}{{\cal L}}
\newcommand{\M}{{\cal M}}
\newcommand{\N}{{\cal N}}
\newcommand{\G}{{\cal G}}
\newcommand{\D}{{\cal D}}
\newcommand{\E}{{\cal E}}
\newcommand{\F}{{\cal F}}
\newcommand{\V}{{\cal V}}
\newcommand{\W}{{\cal W}}
\newcommand{\K}{{\cal K}}
\renewcommand{\H}{{\cal H}}
\newcommand{\OOO}{{\cal O}}
\newcommand{\C}{{\cal C}}
\newcommand{\I}{{\cal I}}
%\renewcommand{\S}{{\cal S}}
\newcommand{\Scal}{{\cal S}}
\newcommand{\Q}{{\cal Q}}
\renewcommand{\P}{{\cal P}}

%%%%
%% lettres mathematiques
%%%%

\newcommand{\maths}[1]{{\mathbb #1}}  
%\newcommand{\maths}[1]{{\bf #1}} 

\renewcommand{\AA}{\maths{A}}
\newcommand{\OO}{\maths{O}}
\newcommand{\RR}{\maths{R}}
\newcommand{\NN}{\maths{N}}
\newcommand{\CC}{\maths{C}}
\newcommand{\QQ}{\maths{Q}}
\newcommand{\BB}{\maths{B}}
\newcommand{\SSS}{\maths{S}}
\newcommand{\DD}{\maths{D}}
\newcommand{\HH}{\maths{H}}
\newcommand{\FF}{\maths{F}}
\newcommand{\KK}{\maths{K}}
\newcommand{\ZZ}{\maths{Z}}
\newcommand{\PP}{\maths{P}}
\newcommand{\XX}{\maths{X}}
\newcommand{\LL}{\maths{L}}
\newcommand{\TT}{\maths{T}}
\newcommand{\UU}{\maths{U}}

%%%%
%% Fonte gothique
%%%%


\newcommand{\aaa}{{\mathfrak a}}
\renewcommand{\ggg}{{\mathfrak g}}
\newcommand{\sss}{{\mathfrak s}}
\renewcommand{\lll}{{\mathfrak l}}
\newcommand{\ooo}{{\mathfrak o}}
\newcommand{\uuu}{{\mathfrak u}}
\newcommand{\vvv}{{\mathfrak v}}
\newcommand{\ppp}{{\mathfrak p}}
\newcommand{\hhh}{{\mathfrak h}}
\newcommand{\fff}{{\mathfrak f}}
\newcommand{\zzz}{{\mathfrak z}}
\newcommand{\CCC}{{\mathfrak C}}
\newcommand{\mmm}{{\mathfrak m}}
\renewcommand{\uuu}{{\mathfrak u}}

%%%%
%% commandes abrevies
%%%%

\newcommand{\noted}[1]{\marginpar{\scriptsize #1}}

\newcommand{\weakstar}{\overset{*}\rightharpoonup}
\newcommand{\ra}{\rightarrow}
\newcommand{\bs}{\backslash}

\newcommand{\ov}[1]{{\overline #1}} 
\newcommand{\wt}[1]{{\widetilde{#1}}}
\newcommand{\wh}[1]{{\widehat{#1}}}


\newcommand{\ga}{\gamma}
\newcommand{\Ga}{\Gamma}



%%%%
%% raccourcis typographiques
%%%%

\newcommand{\semidirect}{{\Bbb n}}
\newcommand{\cqfd}{\hfill$\Box$}

\newcommand{\card}{{\operatorname{Card}}}
\renewcommand{\Re}{{\operatorname{Re}}}
\renewcommand{\Im}{{\operatorname{Im}}}
\newcommand{\Vol}{\operatorname{Vol}}
\newcommand{\Isom}{\operatorname{Isom}}
\newcommand{\codim}{\operatorname{codim}}
\newcommand{\vol}{\operatorname{vol}}
\newcommand{\covol}{\operatorname{Covol}}
\newcommand{\id}{\operatorname{id}}
\newcommand{\Leb}{\operatorname{Leb}}
\newcommand{\PSL}{\operatorname{PSL}}
\newcommand{\SL}{\operatorname{SL}}
\newcommand{\Res}{\operatorname{Res}}
\newcommand{\dvol}{\;d\operatorname{vol}}
\newcommand{\Det}{\operatorname{Det}}
\newcommand{\arcosh}{\operatorname{argcosh}}
\newcommand{\arsinh}{\operatorname{argsinh}}
\newcommand{\axis}{\operatorname{Axis}}
\newcommand{\bigO}{\operatorname{O}}
\newcommand{\smallo}{\operatorname{o}}
\newcommand{\Heis}{\operatorname{Heis}}
\newcommand{\qquadr}{\QQ_{\rm quad}}
\newcommand{\haarheis}{\operatorname{Haar}_{\operatorname{Heis}_3}}

\newcommand{\hdr}{{\HH}^2_\RR}
\newcommand{\htr}{{\HH}^3_\RR}
\newcommand{\hcr}{{\HH}^5_\RR}
\newcommand{\hnr}{{\HH}^n_\RR}
\newcommand{\hnc}{{\HH}^n_\CC}
\newcommand{\hdc}{{\HH}^2_\CC}
\newcommand{\htc}{{\HH}^3_\CC}
\newcommand{\phcr}{\partial_\infty\hcr}


\newcommand{\SLO}{\operatorname{SL}_{2}(\OOO)}
\newcommand{\GLO}{\operatorname{GL}_{2}(\OOO)}
\newcommand{\PSLO}{\operatorname{PSL}_{2}(\OOO)}
\newcommand{\SLOK}{\operatorname{SL}_{2}(\OOO_K)}
\newcommand{\PSLOK}{\operatorname{PSL}_{2}(\OOO_K)}
\newcommand{\SLH}{\operatorname{SL}_{2}(\HH)}
\newcommand{\PSLH}{\operatorname{PSL}_{2}(\HH)}
\newcommand{\SLC}{\operatorname{SL}_{2}(\CC)}
\newcommand{\PSLC}{\operatorname{PSL}_{2}(\CC)}
\newcommand{\SLZ}{\operatorname{SL}_{2}(\ZZ)}
\newcommand{\PSLZ}{\operatorname{PSL}_{2}(\ZZ)}
\newcommand{\SU}{\operatorname{SU}}
\newcommand{\PSU}{\operatorname{PSU}}
\newcommand{\autom}{\operatorname{SU}_f(\OOO_K)}
\newcommand{\Pautom}{\operatorname{PSU}_f(\OOO_K)}
\newcommand{\automH}{\operatorname{SU}_f(\OOO)}
\newcommand{\PautomH}{\operatorname{PSU}_f(\OOO)}
\newcommand{\const}{\iota}
\newcommand{\discr}{\Delta}
\newcommand{\cinfty}{\operatorname{\C_\infty}}
\newcommand{\plane}{\operatorname{\C}}
\newcommand{\SpO}{\operatorname{Sp}_1(\OOO)}
\newcommand{\diam}{\operatorname{diam}}


\newcommand{\tr}{\operatorname{tr}}
\newcommand{\n}{\operatorname{n}}
\newcommand{\Tr}{\operatorname{Tr}}
\newcommand{\Norm}{\operatorname{N}}
\newcommand{\Gal}{\operatorname{Gal}}

\newcommand\Rep{\mathcal R}
\newcommand{\stab}{\operatorname{Stab}}
\newcommand{\flow}[1]{{g^{#1}}}  
\newcommand{\muss}[1]{{\mu^-_{W^{\rm ss}(#1)}}}
\newcommand{\mus}[1]{{\mu^{\rm s}_{#1}}}  
\newcommand{\musu}[1]{{\mu^+_{W^{\rm su}(#1)}}}
\newcommand{\muu}[1]{{\mu^{\rm u}_{#1}}}  
\newcommand{\normal}[1]{\partial^1_{+}{#1}}
\newcommand\oPerp{\operatorname{\wt{Perp}}}
\newcommand\Perp{\operatorname{Perp}}
\newcommand{\curv}{\operatorname{curv}_{\rm S}}
\newcommand\normalout{\partial^1_{+}}
\newcommand\normalin{\partial^1_{-}}
\newcommand\normalpm{\partial^1_{\pm}}
\newcommand\normalmp{\partial^1_{\mp}}

\newcommand\viiva{\medskip
\begin{center}{---------}
\end{center}
\medskip }


%%%%
%% compteurs
%%%%

\newcounter{const}
\newcounter{fig}


%%%%
%% Format de figures
%%%%

\def\myfigure#1#2#3{
%\nopagebreak[3]
\addtocounter{fig}{1}
\[
\begin{array}{c}
\mbox{\psfig{figure=#1.ps,height=#2}}\\
\\ 
\hbox{\rm Figure \arabic{fig} ~: #3.}
\end{array}
\]
}

%% Ne pas oublier d'aller hacker le fichier pstex_t pour remplacer
%% epsfig par psfig

\def\myfigpstex#1#2{
%\nopagebreak[3]
\addtocounter{fig}{1}
\[
\begin{array}{c}
\mbox{\input{#1.pstex_t
}}\\
\\ 
\hbox{\rm Figure \arabic{fig} ~: #2.}
\end{array}
\]
}
